Operational Aspects of C/C++ Concurrency

In this work, we present a family of operational semantics that gradually approximates the realistic program behaviors in the C/C++11 memory model. Each semantics in our framework is built by elaborating and combining two simple ingredients: viewfronts and operation buffers. Viewfronts allow us to express the spatial aspect of thread interaction, i.e., which values a thread can read, while operation buffers enable manipulation with the temporal execution aspect, i.e., determining the order in which the results of certain operations can be observed by concurrently running threads. Starting from a simple abstract state machine, through a series of gradual refinements of the abstract state, we capture such language aspects and synchronization primitives as release/acquire atomics, sequentially-consistent and non-atomic memory accesses, also providing a semantics for relaxed atomics, while avoiding the Out-of-Thin-Air problem. To the best of our knowledge, this is the first formal and executable operational semantics of C11 capable of expressing all essential concurrent aspects of the standard. We illustrate our approach via a number of characteristic examples, relating the observed behaviors to those of standard litmus test programs from the literature. We provide an executable implementation of the semantics in PLT Redex, along with a number of implemented litmus tests and examples, and showcase our prototype on a large case study: randomized testing and debugging of a realistic Read-Copy-Update data structure.

==> 2 <==
\section{Running example: RCU}
\label{sec:rcu-example}

To check adequacy of our semantics against something more interesting and
complex than the litmus tests, we chose RCU (Read-Copy Update)
\cite{McKenney:PhD, McKenney-Slingwine:PDCS98},
which is widely used in the Linux kernel, and so important, that
the consume modifier was introduced in C11 mostly because of it
\cite{rcu-consume}.
RCU is a technique for non-blocking sharing of a linked data structure,
such as a list or a tree, by one writer and multiple readers.
As in \cite{Tassarotti-al:PLDI15},
in this work we concentrate on RCU for a singly linked list,
implemented with QSBR (Quiescent State Based Reclamation)
\cite{Desnoyers-al:TPDS12}.

The central idea of RCU is how the writer treats the data structure.
Instead of in-place modification of a list node,
the writer creates a copy of it, modifies the copy, updates the link
to the node, making the older version inaccessible,
waits until all readers stop using the older version, and reclaims it.

This algorithm doesn't require sequential consistency to be correct,
but relies on a synchronization between the writer and the readers.
On the writer side the aforementioned link update must be performed
by release write, 
whereas the readers must traverse the list performing dereferencing
by read with at least the consume modifier.
The synchronization between the release link update and the consume
dereferencing guarantees that the reader thread can't observe partially
modified nodes.

\subsection{RCU implementation}

A program using QSBR RCU in our language is presented on
Fig.~\ref{fig:rcuProg}.
In the first line there is initialization of thread counters and
a pointer to a list, which is going to be shared between subthreads.
After that there is spawning of three subthreads: a list writer thread
and two list reader threads.

The writer thread appends three values to the list: \lstinline{1},
\lstinline{10}, and \lstinline{100}.
The \lstinline{append} routine consists of 

After that it changes the second value
(\lstinline{10}) to \lstinline{1000}.

%% The writer thread increments \lstinline{cw} counter after updating the list,
%% whereas the readers \lstinline{cr1} and \lstinline{cr2} 

\subsubsection{Language limitations}
Currently, we don't have some essential language constructions such as
memory allocation, variables, and functions, because we didn't need them
for litmus tests we were testing our semantics at. 
There are no fundamental problems of adding them to the language, but
we left it for the near future development because of the lack of time.
Unfortunately, these language limitations affected the RCU example.

Thus, the lack of variables forces us to use acquire reads instead of
consume ones in the \lstinline{traverse} function.
In the function at every \lstinline{repeat} loop iteration we need to
have a pointer to a current list node.
And it has to be provided by a previous iteration
(or by some initialization before the loop for the first iteration).
Because we don't have variables, the only possible way to transfer
the pointer to the next iteration is to store it in some location.
We use \lstinline{curNodeLoc} location for this purpose
in the \lstinline{traverse} function.
Unlike using a variable to store the current node pointer,
writing it to some location and reading it back breaks data-dependency
chain, which is required by consume reads to provide synchronization.
That is why, the reading from \lstinline{rCurNode} location is the acquire one.
Nevertheless, in the example program we can unroll the \lstinline{repeat}
loop three times, because the list contains no more than three entries at
any moment, and use consume reads then.

We don't have explicit memory allocation operation, but 

Finally, even though our language doesn't have functions or macros, and
there are no functions in the actual implementation,
we present the RCU program using them for brevity.

\begin{figure*}
\input{rcuProg}
\caption{The QSBR RCU implementation.}
\label{fig:rcuProg}
\end{figure*}

\app{Add an example of RCU running.}

%% \subsection{Running the RCU in the C11 semantics}
\subsection{RCU in our language}

\app{quiescentState: In actual implementation we put SC modifiers, to reduce
state space and to have better chance not to get in infinite loop.}

\app{Write about consume + RCU, dereferencing of links \etc.}
\app{Say that we can run the RCU example with acquire modifiers, but
have troubles with consume modifiers.
The troubles are that we don't have local variables, so we can't have
a data-dependency chain, which goes through loops.
Unfortunately, we can't solve it by CPS-transformation of the repeat
loop, because the body can be changed by name substitutions.}

\subsection{Dynamic scheduling}
The RCU example is much bigger then litmus tests, which we showed in
the previous sections.
As a result, the state space of the example is tremendous, and it makes
impossible to fully calculate all states by PLT Redex in reasonable time.
The obvious cause of it is high non-determinism of the presented
operational semantics.
\app{Write more about motivation behind the introduced scheduling.
Why can't we just use standard functionality of PLT Redex (like stepper)?}

To circumvent the problem we added a \emph{scheduling}, which evalu layer to the semantics, which makes it deterministic.

So, to be able to check that the example runs in the semantics correctly,
But before we discuss the technical details of scheduling, let's consider that makes
our semantics non-deterministic.

The first reason, obviously, is threads. So, the semantics can make a step for
every thread, which expression hasn't been reduced to $ret\;\mval_{value}$ yet.
The second reason is read actions, which can return any record stored in
a corresponding location history with a time stamp in a range from the viewfront value
to the latest one. The third reason is postponed reads.

Thus, th

\app{Say that our semantics is still non-deterministic because of stuck rules,
but we made it on purpose.}

Thus, the extended state contains a list of \emph{tasks} to perform.
Each task determines 

\app{Say that the state space is too big, so we implemented dynamic
scheduling to be able to run a random path from the state space.

Unfortunately, this approach isn't viable for state spaces with cycles,
because of PLT Redex restrictions. But this problem can be solved by
updating some location in body loop (\eg counter) to avoid state
repetition.

Actually, it isn't a problem, if we will put scheduling history to the state.}


==> Makefile <==
.PHONY: all paper.pdf extended.pdf clean

all: paper.pdf

graph:
	dot -Tps:cairo images/graphMP.dot > images/graphMP.eps

full: graph paper.pdf

paper.pdf: paper.tex defs.tex intro.tex references.bib proceedings.bib llncs.cls *.sty Makefile rcu.tex conclusion.tex related.tex semantics.tex overview.tex implementation.tex appendix.tex discussion.tex summary.tex advanced.tex
	pdflatex paper
	bibtex paper -min-crossrefs=5
	pdflatex paper
	pdflatex paper paper.pdf

extended.pdf: paper.tex defs.tex intro.tex references.bib proceedings.bib llncs.cls *.sty Makefile rcu.tex conclusion.tex related.tex semantics.tex overview.tex implementation.tex appendix.tex discussion.tex summary.tex advanced.tex

	pdflatex --jobname=paper-extended "\def\extflag{}\input{paper}"
	bibtex paper-extended -min-crossrefs=5
	pdflatex --jobname=paper-extended "\def\extflag{}\input{paper}"
	pdflatex --jobname=paper-extended "\def\extflag{}\input{paper}"


clean: 
	rm -f {paper,paper-extended}.{out,dvi,ps,pdf,log} *.{toc,blg,bbl,aux,rel} paper *.log *~ paper.zip *.tar.gz



==> abbrevmap.tex <==
% $Id: abbrevmap.tex,v 1.2 2009-05-14 14:25:57 dimitriv Exp $

\def\dquote{\text{\char'175}}                           % "
\def\lquote{\text{`}}                                   % `
\def\periodi{\PERIOD}                                   % .
\def\periodii{\PERIOD\PERIOD}                           % ..
\def\periodiii{\ldots}                                  % ...
\def\slashEquals{\neq}                                  % /=
\def\twiddleEquals{\cong}                               % ~=
%\def\lessthan{<}                                        % <
%\def\greaterthan{>}                                     % >
\def\equalsGreater{\Rightarrow}                         % =>
\def\equalsEqualsGreater{\Longrightarrow}               % ==>
\def\equalsEqualsEqualsGreater{\Longrightarrow}         % ===>
\def\lessEquals{\Leftarrow}                             % <=
\def\lessEqualsEquals{\Longleftarrow}                   % <==
\def\lessEqualsEqualsEquals{\Longleftarrow}             % <===
\def\lessEqualsGreater{\Leftrightarrow}                 % <=>
\def\lessEqualsEqualsGreater{\Longleftrightarrow}       % <==>
\def\lessEqualsEqualsEqualsGreater{\Longleftrightarrow} % <===>
\def\equalsEquals{\equiv}                               % ==
\def\equalsEqualsEquals{&{}={}&}                        % ===
\def\minusGreater{\to}                          % ->
\def\minusMinusGreater{\longrightarrow}                 % -->
\def\minusPeriodMinusGreater{\dot{\to}}         % -.->
\def\lquoteMinusMinusGreater{\hookrightarrow}           % `-->
\def\minusLittleO{\multimap}                            % -o
\def\minusSlashMinusGreater{\not \to}           % -/->
\def\lessMinus{\gets}                              % <-
\def\lessMinusMinus{\longleftarrow}                     % <--
\def\lessBar{\triangleleft}                             % <|
\def\lessBarGreater{\mathrel{\triangleleft\mspace{-3mu}\triangleright}} % <|>
\def\minusLquote{\rightharpoonup}                       % -`
\def\greaterLess{\times}                                % ><
\def\lessPlusGreater{\oplus}                            % <+>
\def\lessTimesGreater{\otimes}                          % <*>
\def\colon{\COLON}                                      % :
\def\colonColon{\mathbin{\COLON\COLON}}                 % ::
\def\colonColonEquals{\mathbin{\mathord{\COLON}\mathord{\COLON}\mathord{=}}}
                                                        % ::=
\def\semicolon{\mathbin{\SEMICOLON}}                    % ;
\def\justABar{\mathrel{\BAR}}                           % |
\def\barBarMinus{\Vdash}                                % ||-
\def\barEquals{\mathrel{\BAR\mspace{-8mu}\EQUALS}}      % |=
\def\barMinus{\vdash}                                   % |-
\def\minusBar{\dashv}                                   % -|
\def\barMinusMinus#1{\vdash_{#1}}                       % |--
\def\barMinusGreater{\mapsto}                           % |->
\def\barMinusMinusGreater{\longmapsto}                  % |-->
\def\barMinusMinusGreaterGreater{\mapsto\hspace*{-8pt}\to}
                                                        % |-->>
\def\barVeeBar{\Downarrow}                              % |v|
\def\barCircBar{\Uparrow}                               % |^|
\def\barGreater{\triangleright}                         % |>
\def\lessLess{[\![}                                     % <<
\def\lessLessLess{\left[\!\!\left[}                     % <<<
\def\greaterGreater{]\!]}                               % >>
\def\greaterGreaterGreater{\right]\!\!\right]}          % >>>
\def\minusv#1{\using\text{\rulename{#1}}\justifies}     % -----...
%%\def\twiddlei{\TWIDDLE}                                 % ~
\def\twiddlei{\;}                                       % ~
\def\twiddleii{\;}                                      % ~~
\def\twiddleiii{\quad}                                  % ~~~
\def\twiddleiv{\endprooftree\qquad\prooftree}           % ~~~~
\def\twiddlev{\endprooftree\\ \\ \prooftree}            % ~~~~~...
\def\twiddleTwiddleGreater{\rightsquigarrow}            % ~~>
\def\asterisk{\ASTERISK}                                % *
\def\asteriskii{\overline{\ASTERISK}}                   % **
\def\asteriskiii{\dagger}                               % ***
\def\asteriskiv{\star}                                  % ****
\def\asteriskv{\ddagger}                                % *****
\def\plusPlus{\mathbin{\PLUS\hspace*{-4pt}\PLUS}}       % ++
\def\bang{\mathalpha{\BANG}}                            % !
\def\question{\mathalpha{\QUESTION}}                    % ?
\def\slashBackslash{\land}                             % /\

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "modules"
%%% End: 



==> consume.tex <==

\section{Consume Reads: Formal Description}
\label{sec:consume}

% \subsection{Example and Intuition}
% \label{sec:example-intuition}


% \begin{figure}[t]
% \centering 
% \vspace{-.2cm}
%   \begin{tabular}{l@{\ \ \ }l}
%     \begin{minipage}[l]{4.3cm} \small
% \begin{lstlisting}
% |$[$|p|$]_{na}$| := null; |$[$|d|$]_{na}$| := 0; |$[$|x|$]_{na}$| := 0;
% \end{lstlisting}
% \vspace{-.2cm}
% \begin{tabular}{l||l}
% \begin{lstlisting}
% |$[$|x|$]_{rlx}$| := 1;
% |$[$|d|$]_{na}$| := 1;
% |$[$|p|$]_{rel}$| := d
% \end{lstlisting}
% \hspace{.6cm}
% &
% \begin{lstlisting}
% r1 = |$[$|p|$]_{con}$|;
% if   r1 != null
% then r2 = |$[$|r1|$]_{na}$|;
%      r3 = |$[$|x|$]_{rlx}$|
% else r2 = 0; r3 = 0
% fi
% \end{lstlisting}
% \end{tabular}
%     \end{minipage}
% &
%   \end{tabular}
% \caption{An example with a consume read (\textsf{MP\_con+na\_2}).}
% \label{fig:exampleConsume}
% \end{figure}

% % Consume reads are the most subtle part of the C11 standard.  They
% % are used in pair with release writes as well as acquire reads, and
% % also provide some synchronization.

% Unlike \emph{acquire}-reads, \emph{consume}-reads do not update the
% thread's viewfront, but provide a synchronization front only for
% subsequent reads that are dereferencing their result.
 
% Consider the code fragment in Figure~\ref{fig:exampleConsume}.  Here,
% we have message-passing of data stored in \lstinline{d} via location
% \lstinline{p}.  The right thread employs a \emph{consume}-read from
% \lstinline{p}.  In the case when it gets a non-\lstinline{null} value
% (representing a pointer to~\lstinline{d}), it reads from it to
% \lstinline{r2}, and after that from location \lstinline{x} to
% \lstinline{r3}.  There might be three possible outcomes:
% %
% % \is{Why do you
% %   use ``atomic'' brackets for the outcomes?} \app{I don't know that to
% %   use.}
% %
% \lstinline{r1 = null} $ /\ $ \lstinline{r2 = 0} $ /\ $ \lstinline{r3 = 0},
% \lstinline{r1 = d} $ /\ $ \lstinline{r2 = 1} $ /\ $ 
% \lstinline{r3 = 1}, and
% \lstinline{r1 = d} $ /\ $ \lstinline{r2 = 1} $ /\ $ \lstinline{r3 = 0}.
% %
% Changing the consume read to acquire one makes the last triple
%  forbidden, as the right thread's viewfront
% would become up to date with both 
% \lstinline{|$[$|x|$]_{rlx}$| := 1} and \lstinline{|$[$|d|$]_{rlx}$| := 1}
% after acquire-reading a non-\lstinline{null} pointer value from \lstinline{p}.
% %
% At the same time, \emph{consume}-read \lstinline{r1 = |$[$|p|$]_{con}$|}
% provides synchronization only for \lstinline{r2 = |$[$|r1|$]_{rlx}$|},
% which explicitly dereferences its result, but not for
% \lstinline{r3}, which has no data-dependency with it.
% %
% % \is{Yes, please, do, as it currently it doesn't help to appreciate the
% % issue.} \app{Added more description.}

% % \app{Changed.}
% % \is{Okay, what about the next paragraph? Can you give a short and
% %   clean summary of (1) what should be added; (2) how is it going to
% %   make everyone's life better?}
% %
% %% Adding consume reads to the semantics requires
% %% not only changes 
% %% of the state, but also of
% %% the program expression, to be
% %% able to annotate reads affected by a consume one.

% Adding \emph{consume}-reads to the semantics requires us to change the
% program syntax to allow \emph{run-time annotations} on reads, which
% might be affected by consume ones.  When a \emph{consume}-read is
% executed, it retrieves some value/front-entry $(\mvalSubst, \stSigma)$
% from the history, as any other read.  Unlike an \emph{acquire}-read,
% it does not update the thread's viewfront by the retrieved $\stSigma$.
% Instead, it annotates all subsequent data-dependent reads by the
% front~$\stSigma$. Later, when these reads will be executed, they will
% join the front $\stSigma$ from the annotation with the thread's
% viewfront for computing the lower boundary on the relevant location's
% timestamp.  The same process is applied to annotate data-dependent
% postponed reads in buffers, which might refer to the symbolic result
% of a \emph{consume}-read.

% For example, it takes place in load buffering involving

%
%\is{Can you give an example of a postponed read dependency?}

%% Thus, a read, which is data-dependent on a consume one,
%% gets a synchronization

%% \is{I don't understand what do you mean by program representation
%%   level. Was it previously defined?}
%% %
%% Because each read in a program might be affected as
%% \lstinline{r2 = |$[$|r1|$]_{rlx}$|} in the example by one or
%% many previous consume reads, we need to be able to annotate read
%% expressions and postponed read tasks by an additional viewfront each,
%% which contain.
%% \is{Why?}

%% \is{Okay, what about the next paragraph? Can you give a short and
%%   clean summary of (1) what should be added; (2) how is it going to
%%   make everyone's life better?}

%% When the semantics resolves a consume read \is{What do you mean by
%%   resolving a read?}, it takes a value and a synchronization front
%% from the history \is{entry of what? Is it the last one?} entry as in
%% case of acquire read.  After that the front is shrunk to only
%% locations, which are reachable from the value \is{What does it mean -
%%   reachable from the value} by dereferencing, and then it is
%% propagated to read expressions \is{propagated?} and postponed read
%% tasks, which depend on the value. Read actions use these propagated
%% fronts \is{what is this?} as an addition to the thread viewfront, when
%% they are resolved.
%% %
%% \is{Clearly, the paragraph above has to be rewritten in more general
%%   terms, using a simple analogy. How about you say, which dependencies
%%   are tracked in the presence of consume-reads, how they are retrieved
%%   and what they are used for?}

%\item Here, you can also sketch how we do not address the example with
%  two if-s (as it doesn't fit into our ``strictness''-inspired
%  analogy), and why is it considered harmful.

% The following one is irrelevant for the story

% \subsection{Formal Description}
% \label{sec:consumereads}

Unlike \emph{acquire-}reads, which update the thread viewfront, thus
providing synchronization for all subsequent reads in the thread, a
\emph{consume-}read provides the same only for those reads that are
data-dependent from it, \ie, use the result of the \emph{consume-}read
as a location to read from.
%
To account for this effect, we modify several components of the state,
including the syntax of programs, adding the ability to annotate read
operations at runtime with an additional front $\stSigma$, retrieved
by \emph{consume}-reads:
%
\[\begin{array}{rcl}
\RT & ::= & ... \mid \ReadF{\RM}{\locVar}{\stSigma} \mid
             \CasF{\SM}{\FM}{\locVar}{\mvalSubst_{1}}{\mvalSubst_{2}}{\stSigma} 
\\
\stPostOp & ::= & ... \mid read\angled{\vName, \locVar, \RM, \stSigma}
\end{array}\]
%
When an annotated read is resolved, it behaves as an ordinary one, but
it joins the additional front $\stSigma$ with the thread's viewfront
to bound the timestamp of the location to be read.

A consume read, in its turn, when resolved, annotates all subsequent
data-dependent reads in the thread with a retrieved synchronization
front from the history entry: 

{\small{
\[\arrayBlock{
\prooftree
\arrayBlock{
  \auxX = \angled{\stEta, \stPsiRead, ...} \quad ... \quad
  \stEta(\loc, \stTau) = (\mvalSubst, \stSigma) \\
  \auxX' = \angled{\stEta,
    \stPsiRead[\stpath \mapsto \stSigmaRead[\loc \mapsto \stTau]], ...}
}
----------------------------------{ReadCon}
\arrayBlock{
\angled{\EvalContext[\Read{\conM}{\loc}], \auxX} ==> 
\annotateDD{\mvalSubst}{\stSigma}{\stpath}{\angled{\EvalContext[\Ret{\mvalSubst}], \auxX'}}
}
\endprooftree
}\]
}}
%
\noindent
The rule for \emph{consume}-read uses the function $\annotateF$:
\[\arrayBlock{
  ... \\
\angled{\EvalContext[\Read{\conM}{\loc}], \auxX} ==> 
\annotateDD{\mvalSubst}{\stSigma}{\stpath}{\angled{\EvalContext[\Ret{\mvalSubst}], \auxX'}}
}\]

It has four arguments:
\begin{itemize}
  \item $\mvalSubst$ --- a value, read from the history, 
  \item $\stSigma$ --- a front, read from the history,
  \item $stpath$ --- a path, which is the corresponding thread identifier,
  \item and $\angled{\EvalContext[\mvalSubst], \auxX'}$ --- a state pair to be modified
by the function.
\end{itemize}
A result is a modified state pair: $\angled{\EvalContext'[\mvalSubst], \auxX''}$. 

In case the read was an ordinary, \ie, non-\emph{consume}, one the $\mvalSubst$ value
would be propagated to the thread expression, which can be identified by the $\stpath$ path,
by subsequent applying of \ruleF{Subst} rule.
Because the read has \emph{consume} modifier, we not only propagate this value, but
also annotate all reads in $\stpath$-subexpression by $\stSigma$ by applying $\annotateF$
function.
The function also changes $\auxX'$ state component, because it might
update postponed read tasks by the same annotation.




==> discussion.tex <==

\section{Discussion and Future Work}
\label{sec:discussion}

\app{We need to discuss at least these future improvements:}
\begin{itemize}
\item Speculative executions for OTA
\item Postponing writes and read through join point LB\_rlx+join
\item Fences
\item Mutable local variables for RCU
\end{itemize}



==> implementation.tex <==
% \subsection{Tool support}
% \label{sec:tool-support}


%   %% \tickP~means that a test requires a rule of joining threads with
%   %% non-empty operation buffers.
%   %% The rule isn't enabled by default as leading to poor performance.

% The immediate benefit of using Redex is its native support for scoped
% reduction contexts~\cite{Felleisen-Hieb:TCS92}, which we used when
% defining semantics of main term- and viewfront-manipulating rules.
% %
% Furthermore, PLT Redex provides convenient machinery for
% \emph{tracing} program evaluation and \emph{stepping} through the
% execution traces~\cite[\S 15]{Felleisen-al:Redex}, which proved to be
% invaluable for first debugging the semantics itself and then using the
% implementation to debug large case studies (\cf
% Section~\ref{sec:rcu-example}).
% %
% The only problem we encountered is when extending specific transition
% rules and meta-functions for dealing with enhanced program state. This
% issue has been solved using Racket's native support for
% macro-expansions.


% \begin{itemize}[leftmargin=*]

% \item Why we decided to use the PLT
%   Redex~\cite{Klein-al:POPL12,Felleisen-al:Redex};

% \item Where to get the prototype;\footnote{\url{https://github.com/anlun/OperationalSemanticsC11}}

% \item What are the core components and how they are inherent to all
%   instantiations with different constructs;

% \item An example of a specific combination of features, delivering a
%   complete semantics;

% \item Perhaps, a couple of sentences on hacks that were made in order
%   to make everything work together (\eg, the stuff with macros).

% \end{itemize}


==> iriw.tex <==
\noindent Data from the operational semantics ($\exod$):\\
\noindent\mbox{\quad} $\textit{threads} = \{ 0,\ 1,\ 2,\ 3,\ 4 \}$\\
{\renewcommand{\raiseaction}[1]{\mbox{#1}}
\noindent\mbox{\quad} $\textit{actions} =$\\
 \mbox{\quad\quad} Thread $0: \{\WA{a}{na}{x}{0},\ \WA{b}{na}{y}{0}\}$\\
 \mbox{\quad\quad} Thread $1: \{\WA{c}{rel}{x}{1}\}$\\
 \mbox{\quad\quad} Thread $2: \{\WA{d}{rel}{y}{1}\}$\\
 \mbox{\quad\quad} Thread $3: \{\RA{e}{acq}{x}{1},\ \RA{f}{acq}{y}{0}\}$\\
 \mbox{\quad\quad} Thread $4: \{\RA{g}{acq}{y}{1},\ \RA{h}{acq}{x}{0}\}$\\
}
\noindent\mbox{\quad} $\textit{location-kinds} = \{x \mapsto \textsc{Atomic},\ y \mapsto \textsc{Atomic}\}$\\
\noindent\mbox{\quad} \textit{sequenced-before} $\ttran{sb} = \{$ $a \ttran{} b$,\ $e \ttran{} f$,\ $g \ttran{} h$ $\}$\\
\noindent\mbox{\quad} \textit{data-dependency} $\ttran{dd} = \{$  $\}$\\
\noindent\mbox{\quad} \textit{control-dependency} $\ttran{cd} = \{$  $\}$\\
\noindent\mbox{\quad} \textit{additional-synchronized-with} $\ttran{asw} = \{$ $b \ttran{} c$,\ $b \ttran{} d$,\ $b \ttran{} e$,\ $b \ttran{} g$ $\}$\\
\noindent Existential witness data ($\exed$):\\
\noindent\mbox{\quad} \textit{reads-from} $\ttran{rf} = \{$ $a \ttran{} h$,\ $b \ttran{} f$,\ $c \ttran{} e$,\ $d \ttran{} g$ $\}$\\
\noindent\mbox{\quad} \textit{SC-order} $\ttran{sc} = \{$  $\}$\\
\noindent\mbox{\quad} \textit{modification-order} $\ttran{mo} = \{$ $a \ttran{} c$,\ $b \ttran{} d$ $\}$\\
\noindent\mbox{\quad} \textit{lock-order} $\ttran{lo} = \{$  $\}$\\
\noindent\mbox{\quad} \textit{a-order} $\ttran{ao} = \{$  $\}$\\
\noindent\mbox{\quad} \textit{total-order} $\ttran{tot} = \{$  $\}$\\
\noindent Derived relations:\\
\noindent\mbox{\quad} \textit{happens-before} $\ttran{hb} = \{$ $a \ttran{} b$,\ $a \ttran{} c$,\ $a \ttran{} d$,\ $a \ttran{} e$,\ $a \ttran{} f$,\ $a \ttran{} g$,\ $a \ttran{} h$,\ $b \ttran{} c$,\ $b \ttran{} d$,\ $b \ttran{} e$,\ $b \ttran{} f$,\ $b \ttran{} g$,\ $b \ttran{} h$,\ $c \ttran{} e$,\ $c \ttran{} f$,\ $d \ttran{} g$,\ $d \ttran{} h$,\ $e \ttran{} f$,\ $g \ttran{} h$ $\}$\\
\noindent\mbox{\quad} \textit{visible-side-effect} $\ttran{vse} = \{$ $a \ttran{} h$,\ $b \ttran{} f$,\ $c \ttran{} e$,\ $d \ttran{} g$ $\}$\\
\noindent\mbox{\quad} \textit{inter-thread-happens-before} $\ttran{ithb} = \{$ $a \ttran{} c$,\ $a \ttran{} d$,\ $a \ttran{} e$,\ $a \ttran{} f$,\ $a \ttran{} g$,\ $a \ttran{} h$,\ $b \ttran{} c$,\ $b \ttran{} d$,\ $b \ttran{} e$,\ $b \ttran{} f$,\ $b \ttran{} g$,\ $b \ttran{} h$,\ $c \ttran{} e$,\ $c \ttran{} f$,\ $d \ttran{} g$,\ $d \ttran{} h$ $\}$\\
\noindent\mbox{\quad} \textit{synchronized-with} $\ttran{sw} = \{$ $b \ttran{} c$,\ $b \ttran{} d$,\ $b \ttran{} e$,\ $b \ttran{} g$,\ $c \ttran{} e$,\ $d \ttran{} g$ $\}$\\
\noindent\mbox{\quad} \textit{release-sequence} $\ttran{rs} = \{$ $c \ttran{} c$,\ $d \ttran{} d$ $\}$\\
\noindent\mbox{\quad} \textit{hypothetical-release-sequence} $\ttran{hrs} = \{$ $c \ttran{} c$,\ $d \ttran{} d$ $\}$\\
\noindent\mbox{\quad} \textit{dependency-ordered-before} $\ttran{dob} = \{$  $\}$\\
\noindent\mbox{\quad} \textit{carries-a-dependency-to} $\ttran{cad} = \{$  $\}$\\
\noindent\mbox{\quad} \textit{unsequenced_races} $\ttran{ur} = \{$  $\}$\\
\noindent\mbox{\quad} \textit{data_races} $\ttran{dr} = \{$  $\}$\\
\noindent\mbox{\quad} \textit{indeterminate-reads} (ir) = \{\}\\
\noindent\mbox{\quad} \textit{locks-only-bad-mutexes} (locks_only_bad_mutexes) = \{\}\\



==> oldText.tex <==
%% With additional axiom mentioned above a semantics of program with only \seqCst~memory operations
%% is the same as if it is executed in sequential consistent memory model settings. Thus, in latter model
%% a state is usually presented by a partial function ($\stEta$) from a location ($\loc$)
%% to a value ($\mval$). We have
%% mostly the same thing, if we change codomain of that function to a set of pairs $(\stTau, \mval)$,
%% where $\stTau$ is a timestamp, which is unique in a set. When $\mval$ from the pair with the last
%% $\stTau$ is a current value, corresponding to the location. This representation is a \emph{history}
%% of location changes.

%% At this layer the $\auxX$ component of the state consists of two elements: $\stEta$
%% and $\stSC$. The $\stEta$ element is a generalized heap, or \emph{history}.
%% A history $\stEta$ is a function from a location $\loc$ to a set of \emph{writes} to this location.
%% Every location write is a triple of the form $(\stTau, \mval, \stSigma)$, where $\stTau$ is
%% a unique for the location timestamp, $\mval$ is a corresponding write value, and $\stSigma$ is a
%% front discussed later. Graphically history can be presented as a table, where columns corresponds
%% to locations and rows corresponds to timestamps.

%% \begin{tabular}{r|c|c}
%%   & x  & y \\
%%   \hline
%% 0 & $(1,\stSigma_{x0})$ & $(2, \stSigma_{y0})$ \\
%% 1 & $(15, \stSigma_{x1})$ & - \\
%% 2 & $(39, \stSigma_{x2})$ & -
%% \end{tabular}

%% \app{Write more about this example.}

%% A $\stSigma$ ranges \emph{fronts}. A front is a partial function from a location to a timestamp.
%% In most cases $\stSigma(\loc)$ is used to denote the lower timestamp, which can be used by someone
%% (\eg a thread) to read a value of $\loc$ from $\stEta$.
%% The $\stSC$ element of a state maps $\loc$ to a timestamps, which where \emph{visible} for a thread
%% performed last \seqCst~operation, after this operation.
%% In case of a language with only \seqCst~operations, $\stSC$ points to last write in the history for every
%% location in it. 

%% In this layer we are able to use just ordinary heap (a partial function from locations to values),
%% but we use a pair $(\stEta, \stSC)$, because it extends in other layers.

%% \app{Put here rules for SC operations.}

%In the formalization \cite{Batty-al:POPL11} of C11 memory model, which we use as a reference
%and refer later as C11 memory model or just C11,
%the most important relation between memory actions is \happensBefore~relation.
%This relation is a generalization of an strict total order on actions in sequential consistent
%models. It isn't transitive in C11, but it is in a subset of C11 without \emph{consume} operations.
%At this point we assume this subset of C11.
%In these restrictions the \happensBefore~is a transitive closure of a natural inter-thread
%order on actions, \synchronizedWith~relation, that relates release writes and acquire reads
%if they are related by \readFrom, and a relation between fork/join actions and first/last actions
%of corresponding threads.
%An intuition behind the \happensBefore~relation is that
%if $\alpha_1$ action is \happensBefore~$\alpha_2$ action, then
%$\alpha_2$ sees a result of $\alpha_1$ as well as results of actions, that
%\happensBefore~$\alpha_1$.

%Also, there is an axiom \emph{consistent\_modification\_order}.
%It states that there is a strict total order over all write actions at each atomic location, and
%this order is consistent with \happensBefore~relation. It doesn't state an existence of
%a similar strict total order over writes at non-atomic locations, but they are totally ordered by
%the \happensBefore~relation in consistent executions,
%because if they aren't, then an execution contains a data race on non-atomics. 

%In our semantics we don't distinguish non-atomic and atomic locations, and every
%location can be manipulated by non-atomic and atomic operations. But our semantics identifies
%data races on non-atomic operations.

%As discussed above for consistent executions we can
%assume that all write actions are each location is totally
%ordered, and the order respects the \happensBefore~relation.
%That makes possible to enumerate writes
%for each location. This observation is used in our semantics to represent a heap in a generalized way.
%We call it a \emph{history} ($\stEta$). It is a partial map 
%$\StIota \times \StTau \rightharpoonup \StMu \times \StSigma$, where $\StIota$ is a set of locations,
%$\StTau$ is a set of \emph{timestamps} (isomorphic to $\mathbb{N}_0$),
%$\StMu$ is a set of \emph{values}, which can be stored in locations,
%and $\StSigma$ is a set of \emph{fronts}. A notion of fronts is discussed below.
%Here, timestamps are used to enumerate writes.
%A history is \emph{prefix closed} for every location --- if $\stEta(\stIota, \stTau)$ is defined,
%then $\stEta(\stIota, \stTau')$ is defined for every $\stTau' \leq \stTau$.
%An execution of a write action 


==> stateTraceFig.tex <==
%% \begin{figure}[t]
\cntrd{
  \stateTbl[2pt]{\floc}{\dloc}{
\tauFst & \emptyCell{|} & \emptyCell{} \\
\stateTblEmptyLine

\stateLabel{Step 1: \commandInline{01emp} by the parent thread.}
\tauFst & 0, \emptyFront \hfill \parentFrontMark
        & \emptyCell{} \\
\stateTblEmptyLine

\stateLabel{Step 2: \commandInline{02emp} by the parent thread.}
\tauFst & 0, \emptyFront \hfill \parentFrontMark
        & 0, \emptyFront \hfill \parentFrontMark \\
\stateTblEmptyLine

\stateLabel{Step 3: subthreads spawn.}
\tauFst & 0, \emptyFront \hfill \leftFrontMark \rightFrontMark
        & 0, \emptyFront                \hfill \leftFrontMark \rightFrontMark \\
\stateTblEmptyLine

\stateLabel{Step 4: \commandInline{03emp} by the left subthread.}
\tauFst & 0, \emptyFront \hfill \leftFrontMark \rightFrontMark
        & 0, \emptyFront \hfill \rightFrontMark \\
\tauSnd & \emptyCell{|}
        & 5, \emptyFront \hfill \leftFrontMark \\
\stateTblEmptyLine

\stateTblTextLine{p{\linewidth}}{
\emph{NB:} A write operation updates thread viewfront
(here \redsq~marker on \dloc\ from \tauFst~to \tauSnd),
because a thread becomes aware of its own writes right away.
}
\stateTblEmptyLine

\stateLabel{Step 5: \commandInline{04} by the left subthread.}
\tauFst & 0, \emptyFront \hfill \rightFrontMark 
        & 0, \emptyFront                \hfill \rightFrontMark \\
\tauSnd & 1, (\floc\ $\smapsto$ \tauSnd, \dloc\ $\smapsto$ \tauSnd) \hfill \leftFrontMark
        & 5, \emptyFront                                          \hfill \leftFrontMark \\

\stateTblTextLine{c}{...}
\stateTblTextLine{l}{The right subthread gets 0s by \commandInline{05} in the loop.}
\stateTblTextLine{c}{...}

\stateLabel{Step 6: the right subthread becomes aware of \floc\ $\smapsto$ \tauSnd.}
\tauFst & 0, \emptyFront
        & 0, \emptyFront            \hfill \rightFrontMark \\
\tauSnd & 1, (\floc\ $\smapsto$ \tauSnd, \dloc\ $\smapsto$ \tauSnd)
             \hfill \leftFrontMark \rightFrontMark
        & 5, \emptyFront                                  \hfill \leftFrontMark \\
\stateTblEmptyLine

\stateLabelP{Step 7: the right subthread reads 1 from \floc\ and
                     synchronizes its viewfront with one
                     located in the corresponding \floc\ record. \newline
             (\floc\ $\smapsto$ \tauSnd, \dloc\ $\smapsto$ \tauFst)
             $\lub$ (\floc\ $\smapsto$ \tauSnd, \dloc\ $\smapsto$ \tauSnd)
             = (\floc\ $\smapsto$ \tauSnd, \dloc\ $\smapsto$ \tauSnd)}
\tauFst & 0, \emptyFront
        & 0, \emptyFront \\
\tauSnd & 1, (\floc\ $\smapsto$ \tauSnd, \dloc\ $\smapsto$ \tauSnd)
             \hfill \leftFrontMark \rightFrontMark
        & 5, \emptyFront
             \hfill \leftFrontMark \rightFrontMark \\

\stateTblTextLine{c}{...}
\stateTblTextLine{l}{The right subthread reads the latest value of \dloc\ (5).}
\stateTblTextLine{c}{...}

\stateLabelP{Step 8: subthreads join} 
\tauFst & 0, \emptyFront
        & 0, \emptyFront \\
\tauSnd & 1, (\floc\ $\smapsto$ \tauSnd, \dloc\ $\smapsto$ \tauSnd)
             \hfill \parentFrontMark
        & 5, \emptyFront
             \hfill \parentFrontMark \\
  }
}

%% \caption{An evaluation of a heap history}
%% \label{tbl:histEx}
%% \end{figure}


==> syntacticRules.tex <==
\begin{figure*}[t]\small
\centering
{
\small{
\[\begin{array}{c}
\prooftree
----------------------------------{Subst}
\angled{\EvalContext[\Bind{\vName}{\Ret{\mvalSubst}}{\AST}], \auxX} ==> 
\angled{\EvalContext[\AST[\vName \leftarrow \mvalSubst]], \auxX}
%
~~~~~
%
\Number~\neq~0
----------------------------------{If-True}
\arrayBlock{
  \angled{\EvalContext[\IfThenElse{\Number}{\AST_{1}}{\AST_{2}}], \auxX} ==>
  \angled{\EvalContext[\AST_{1}]], \auxX}
}
%
~~~~~
%
----------------------------------{If-False}
\arrayBlock{
  \angled{\EvalContext[\IfThenElse{0}{\AST_{1}}{\AST_{2}}], \auxX} ==>
  \angled{\EvalContext[\AST_{2}]], \auxX}
}
%
~~~~~
%
\vName \text{ -- fresh invariable}
----------------------------------{Repeat-Unroll}
\arrayBlock{
  \angled{\EvalContext[\Repeat{\AST}], \auxX} ==>
  \angled{\EvalContext[\Bind{\vName}{\AST}
                 {\IfThenElse{\vName}{\Ret{\vName}}
                              {\Repeat{\AST}}}],
            \auxX}
}
%
~~~~~
%
\auxX' = \spawn{\EvalContext}{\auxX}
----------------------------------{Spawn}
\angled{\EvalContext[\Spw{\AST_{1}}{\AST_{2}}], \auxX} ==>
\angled{\EvalContext[\Par{\AST_{1}}{\AST_{2}}], \auxX'}
%
~~~~
%
\auxX' = \joinP{\EvalContext}{\auxX}
----------------------------------{Join}
\angled{\EvalContext[\Par{\Ret{\mvalSubst_{1}}}{\Ret{\mvalSubst_{2}}}], \auxX} ==>
\angled{\EvalContext[\Ret{\Pair{\mvalSubst_{1}}{\mvalSubst_{2}}}], \auxX'}
%
~~~~~
%
---------------------------------{Choice-Fst}
\arrayBlock{
  \angled{\EvalContext[\EvalEUContext[\Choice{~\Expr_{1}}{\Expr_{2}}]], \auxX} ==> %\\
  \angled{\EvalContext[\EvalEUContext[\Expr_{1}]], \auxX}
}
%
~~~~
%
----------------------------------{Choice-Snd}
\arrayBlock{
  \angled{\EvalContext[\EvalEUContext[\Choice{~\Expr_{1}}{\Expr_{2}}]], \auxX} ==> %\\
  \angled{\EvalContext[\EvalEUContext[\Expr_{2}]], \auxX}
}
\endprooftree
\end{array}\]
}}
\caption{The core rules of the semantics.}
\label{fig:basic-sem}
\end{figure*}

